Daisen: A Framework for Visualizing Detailed GPU Execution

Graphics Processing Units (GPUs) have been widely used to accelerate artificial intelligence, physics simulation, medical imaging, and information visualization applications. To improve GPU performance, GPU hardware designers need to identify performance issues by inspecting a huge amount of simulator-generated traces. Visualizing the execution traces can reduce the cognitive burden of users and facilitate making sense of behaviors of GPU hardware components. In this paper, we first formalize the process of GPU performance analysis and characterize the design requirements of visualizing execution traces based on a survey study and interviews with GPU hardware designers. We contribute data and task abstraction for GPU performance analysis. Based on our task analysis, we propose Daisen, a framework that supports data collection from GPU simulators and provides visualization of the simulator-generated GPU execution traces. Daisen features a data abstraction and trace format that can record simulator-generated GPU execution traces. Daisen also includes a web-based visualization tool that helps GPU hardware designers examine GPU execution traces, identify performance bottlenecks, and verify performance improvement. Our qualitative evaluation with GPU hardware designers demonstrates that the design of Daisen reflects the typical workflow of GPU hardware designers. Using Daisen, participants were able to effectively identify potential performance bottlenecks and opportunities for performance improvement. The open-sourced implementation of Daisen can be found at gitlab.com/akita/vis. Supplemental materials including a demo video, survey questions, evaluation study guide, and post-study evaluation survey are available at osf.io/j5ghq.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> ieeevis_review.tex <==
Reviewer 2 (Primary Reviewer)

Paper type

System
Expertise

Knowledgeable
Overall Rating

<b>3 - Possible Accept</b><br/> The paper is not acceptable in its current state, but might be made acceptable with significant revisions within the conference review cycle.<br/>If the specified revisions are addressed fully and effectively I may be able to return a score of '4 - Accept'.
Supplemental Materials

Acceptable
Justification

The Daisen system is well described and includes several useful elements. The utility of a system like this is established in the preliminary material and the overall system architecture are thoroughly described. On the minus side, I'm not convinced they have matched all of their own design criteria. I also don't see reference to other standard works that are int eh same design space as some of their contributions. I'm left wondering how this is better and if they have data to effectively argue that position. Therefore, I'm left feeling like this is a good description of their system with strong anecdotal evidence, but lacking in a true evaluation.
The Review

The overall system goal is to help GPU hardware designers understand how their design choices impact the execution of benchmark programs through trace recordings in simulators. The claim is that existing systems are insufficient because they are either (1) proprietary (thus not extensible), (2) tightly tied to specific simulators or (3) too complex with many tightly focused tools, requiring new custom views for each new GPU subsystem type.

Daisen presents a plausible generic solution for GPU data collection and presentation. Along with this, it presents useful/informative task analysis and set of task abstractions.

This paper walks through the GPU concepts nicely. It does a good overview of the specific vocabulary used in GPU hardware design and software concepts. The coordination of hardware and software concepts continues throughout the paper. This makes it easier to read and re-enforces that the problem space is in the transition between the two. There is a well-done discussion of cross-context reasoning in section 7.3, how both hardware and software concepts are displayed, and then how they are kept aligned.

Though Daisen is targeted at GPU designers, it is clear that the problem is how designs impact issues that express themselves in the software layer. It is also makes it clear that some of the work in Daisen may help software developers understand the GPU behavior (even if from a simulator) and thereby help them develop a better understanding of the GPU behavior their code might induce. 

The discussion about design requirements starts off in a fairly common fashion, with 'functional' requirements. However, the non-functional requirements discussion is worth mention. Even though it is short (3 paragraphs in section 5), it helps detail the operational context that Daisen will be used in. Though the multi-person analysis is not well fleshed out in the rest of the paper (mentioned a few times for how it could be done, but not really why it might be done), the idea of analysis bookmarking is one that could be used in many other projects.

I was surprised by the claim that the generic metrics are at least sometimes equivalent (as made in section 7.2) and skeptical at first. However, the claim is backed up by the user experience reports later in the paper. It would be nice if this was explored more, as the paper's claims are very expansive while the experience report only gives one person's impression. However, it is good to see the paper's claim is not entirely ad-hoc.

I am left with several questions:
* How does this task analysis compare to CPU task analysis? Are the concepts similar enough that they could be applied in a CPU concept, or is it strictly GPU? The data abstraction seems generic enough, and the functional units concepts have analogs though the scales would be different.
* Why did they develop their own trace format? What did they find lacking with formats like otf, vtf or slog2? Thought these other formats were designed for HPC applications, they solve many of the same problems (especially otf). 

The data abstraction discussion is difficult to follow. It would be easier to follow if there were an example sequence of entries for a pair of locations (say a compute and memory unit). How does the memory request look on both haves of that system? What does the completion look like? The examples in table 2 are useful to understand the meaning of individual fields, but the overall sequence is hard to follow in the text.

The overview visualization seems useful only for verification. It seems like it might even hinder discovery since there are pages and pages of simple diagrams and search is by name. The authors claim that it supports task FR-3, but makes indication how lots of small multiples spread over many pages gives a good overview of system behavior or helps a designer discern sub-nanosecond behaviors from millisecond level traces. There is a plausible path to selection through the search capabilities, but discovery is more complicated and currently appears to be based on the designer's ability to effectively select plausible components and remember trends across pages. 

In the end, the uniqueness and utility of visualizations seem over-claimed as contributions. On the other hand, the system architecture and exploration of the operational context seems like a solid contributions.


Typos:
Section 7.4 refers to "NRF" when it should be "NFR"
Summary Rating

<b>Possible Accept</b><br/> The paper is not acceptable in its current state, but might be made acceptable with significant revisions within the conference review cycle.<br/>If the specified revisions are addressed fully and effectively I may be able to return a score of '4 - Accept'.
The Summary Review

This paper presents some interesting work on GPU visualization. Overall this work is moving in a promising direction and may have a significant contribution at this time. However, there are significant questions left open by the paper and as such is not quite ready for acceptance at InfoVis this year. 

We provide some guidance below to improve the writing and better situate the work in the context of existing work on performance visualization, that we hope are helpful to you in resubmitting the work to a future venue.


* A more complete treatment of the general performance visualization literature. This should include existing work in for both CPUs and GPUs. This is necessary to contextualize this paper with existing work.
* More discussion/detail of the data collection and analysis for the task abstraction *in the paper* (rather than the supplemental material). This is one of the paper's strengths that may be transferred to other work, but is currently insufficiently described to facilitate that transfer.
* A critique of the existing data formats, indicating why existing formats were insufficient for DAISEN's task, such that they developed a new one. This is necessary to validate their claim of contributing a useful data format.
* The user evaluation setup is too summarized to assess its contribution. The participants background and quantity are not well enough described to assess if they are a representative group. The dataset used is not well described either. What is in it? How large is it? Is it one of the datasets used in demonstration materials?
* The discussion of the user evaluation is fairly generic. As the authors point out, the large number of execution elements is a defining trait in GPU architectures. What was the impact of DAISEN on that issue?
* The authors claim generalizability of their system to other simulators and to live-monitoring. However, the evidence presented is fairly narrow. Evidence for generalizability such as application to another simulator, use on a task with a distinct workflow or a more detailed discussion the impact of live-streaming would be important.
Second round comments (public)

(blank)
Second round supplementary materials comments

(blank)
Reviewer 3 (Secondary Reviewer)

Paper type

Application / Design Study
Expertise

Knowledgeable
Overall Rating

<b>3 - Possible Accept</b><br/> The paper is not acceptable in its current state, but might be made acceptable with significant revisions within the conference review cycle.<br/>If the specified revisions are addressed fully and effectively I may be able to return a score of '4 - Accept'.
Supplemental Materials

Not acceptable
Justification

This paper is a design study for performance analysis of GPU hardware design. Among its strengths are the clear, well-abstracted background section and consulting a large number off GPU hardware designers to create a clear, detailed task abstraction. However, there’s little information in the paper about how the backing data led to it. The design seems clean and I generally believe the design will be useful, though I’m not convinced the evaluation supports that. It’s unclear who performed the case studies (are they usage scenarios instead?) In the Section 9 evaluation, it was unclear what kind of datasets were explored by the users. These are not described. How realistic were they and how similar to the training/demo data? The results are so summarized it was hard for me to understand what the participants did. It may be helpful to go into more detail about what participants did rather than having usage scenarios.

It’s also not clear what the greater visualization community should take from this study. The design isn’t explained in context of other performance visualizations (there is significant missing related work) and there are no reflections on the design study itself.

I chose “not acceptable” for the supplemental material because I was unable to view most of it. Rather than uploaded, it was placed behind a bit.ly link. These links do referrer tracking and can be changed after the submission deadline. For anonymity and fairness, I did not follow the link. Also, due to its size and having “osf” in the name, I initially confused it for an osf.io link, but caught myself before following. There is one movie attached however which is very well done and I support its inclusion.
The Review

Expanding on the justification, I was excited by the task abstraction due to the wide sourcing of the data and the use of the hierarchical approach. The resulting task hierarchy and requirements seem reasonable, butI would have liked to know more about what was asked by participants. This might have been in the unreviewable supplemental material, but the paper should also stand on its own. More detail here would be useful—someone running their own design study could learn what worked in terms of surveying domain experts in terms of what was asked, how to elicit responses, etc. It would be nice to know how consistent the responses were and how many responses supported each tasks.

There’s a significant amount off missing related work to the point where the paper makes design claims that are inconsistent with the literature. There’s missing directly related work in GPU performance visualization [1]. Furthermore, the paper makes a point that CPU performance visualizations are single-threaded. This is unaware of a large body of work in performance analysis for parallel computing [2]. In particular, there’s been a long history of nesting to compress the call chain (e.g., in our community, PerfOpticon [3] categorically and Ravel [4] grayscale ramp) and laying out entities/tasks to fit rather than fixed to rows [5]. The claims made by the paper that tasks are usually visualized one per row, based on TraceVis (page 6), is not consistent with these other works.

For the case studies, who performed the case studies (domain experts?) and were these known problems?

For the evaluation, what was the dataset that was used by the participants? Were any participants involved in the design? How similar was it to the demonstration dataset? What was the scale? Perhaps one of the case studies could walk through how a participant approached the evaluation session. As the paper is written, there is little information on what was done. It is highly summarized.

The evaluation design does seem rich, with real domain experts and 90 minutes of time, but the information given in the paper is presently insufficient to fully evaluate the evaluation. It’s hard to understand the limitations of the evaluation because of this.

In summary, I recommend this paper:
* Expand discussion of the task analysis survey and support for tasks
* Expand related work to include other performance visualization in parallel contexts closer to this domain
* Expand explanation of the evaluation, in particular illustrate how the participants interacted with the system
* Decrease case studies to support the above expansion, especially if they are not performed by experts, and be more clear about the context in which they are performedd
* Since the limitations are focused only on the task analysis, they should be moved to that section.



Other comments:

I really liked the background section. I thought it was succinct, clear, and included just the right amount of information.

The movie is clear and well-paced.


References:
[1] Rosen, P. (2013), A Visual Approach to Investigating Shared and Global Memory Behavior of CUDA Kernels. Computer Graphics Forum, 32: 161-170. doi:10.1111/cgf.12103

[2] http://hdc.cs.arizona.edu/people/kisaacs/STAR/

[3] Moritz, D., Halperin, D., Howe, B. and Heer, J. (2015), Perfopticon: Visual Query Analysis for Distributed Databases. Computer Graphics Forum, 34: 71-80. doi:10.1111/cgf.12619

[4] K. E. Isaacs et al., "Combing the Communication Hairball: Visualizing Parallel Execution Traces using Logical Time," in IEEE Transactions on Visualization and Computer Graphics, vol. 20, no. 12, pp. 2349-2358, 31 Dec. 2014, doi: 10.1109/TVCG.2014.2346456.

[5] W. De Pauw, J. Wolf and A. Balmin, "Visualizing jobs with shared resources in distributed environments," 2013 First IEEE Working Conference on Software Visualization (VISSOFT), Eindhoven, 2013, pp. 1-10, doi: 10.1109/VISSOFT.2013.6650535.
Reviewer 1 (External Reviewer)

Paper type

Application / Design Study
Expertise

Knowledgeable
Overall Rating

<b>3.5 - Between Possible Accept and Accept</b><br/>
Supplemental Materials

Acceptable
Justification

The paper presents a visualization for GPU performance evaluation with consideration of generalizability. Their work also provides a comprehensive process from the design to the evaluation of their visualization, including task analysis, identification of requirements, and the user study. The paper is generally well written and their approach seems convincing for this application target. However, I have concerns about the lack of novelty in visualizations and insufficient solutions to address the problems specific to GPU performance analysis (e.g., the scalability problem). Thus, I rate this paper with a score of 3.5.
The Review

This paper presents a visualization framework for analyzing GPU performance obtained via GPU simulators. The paper is well-written and provides all the important components to design and evaluate their framework (e.g., task analysis and user study). I have one major concern in their visualization design/contributions. 

[Limitations of their visualization design]
They visualize the performance metrics, tasks, etc. with the straightforward/traditional plots, such as line charts. As this work can be considered as an “application/design study” paper, this is acceptable. However, I feel the authors should have addressed the problems specific to GPU performance analysis. As the authors discussed, the major difference between CPU and GPU performance analyses is the massiveness of GPU computation. As a result, the visual scalability issue would easily occur. For example, as stated in Sec. 7.1, while there could be thousands of components, the framework addresses this problem only by using multiple web pages and the regular expression based filtering. In this way, the GPU designer would be able to find their expected bottlenecks (because they know which components they should review) but it is difficult to find unexpected bottlenecks. For example, the authors could provide some algorithmic support to help find related metrics to the bottlenecks. Also, the current example of the component view shows 3-6 wavefronts but there could be more. In such a case, from the hierarchically packed rectangles, it would be difficult to see sublayers. A similar problem can occur in the color-coding of tasks based on the category and action. Is the number of (categories x actions) generally small? If not, using colors also has a scalability issue.

[Other (minor) problems]
- Sec. 2: I would like to see Fig. 2 on page 2 to read the content with the figure.
- Table 1: Even though "component" is one of the most important key concepts, the authors do not provide a sufficient description in Sec. 2.
- Sec. 4: "open coded" => "open-coded"
- Sec. 6: "We define … as a task (see Table 2)." => I was confused about the relationship between "task" and Table 2 at this sentence. Probably, "... as a task. As listed in Table 2, each task is assigned …."
- Sec. 7: "including the Overview Panel, the component view, and the Task View" => the component view should be capitalized as well.
- Sec. 8.2 and Fig. 9: How can we compare the difference between multiple runs? Is there any special support for the comparison? or just using two browser windows? 
- Sec. 9 and Fig. 10: Are there any reasons that "Identify hardware …" and "Examine software ..." got relatively lower scores than other tasks?

"Revisions Required"
- addressing (minor) problems listed above
- at least, discussing the limitations of the current visualization design and the potential solutions. 
Reviewer 4 (External Reviewer)

Paper type

Application / Design Study
Expertise

Knowledgeable
Overall Rating

<b>3.5 - Between Possible Accept and Accept</b><br/>
Supplemental Materials

Acceptable
Justification

Summary: This paper proposes a visualization tool Daisen for monitoring the performance of GPUs and identifying bottleneck issues. An effective data collection library has been designed to gather data from the GPU architecture which is implemented for a generic simulator framework. The postmortem trace analysis data is then fed into the visualization subsystem through a MySQL database. There is an overview visualization for execution traces of different components as small multiples, and a composite view of task view, component view, and legend bar. The composite view supports examining the usage of the GPUs in a hierarchical fashion, between GPU threads to the instruction. The composite view is effective in identifying #wavefronts executing in parallel in a compute unit at any given point in time. The lesser #wavefronts implies bottlenecks, and the tool helps in exploring the hierarchy to identify where improvement is needed. The tool is quite useful for hardware engineers to track the performance of the GPUs in today’s ever-increasing presence of GPUs in computational applications. To my knowledge, there are no other such comprehensive tools. The demo video and the user study demonstrate the intuitive usability of the tool.

This design study is complete and well-presented. Hence, my rating for acceptance.
The Review

Summary: This paper proposes a visualization tool Daisen for monitoring the performance of GPUs and identifying bottleneck issues. An effective data collection library has been designed to gather data from the GPU architecture which is implemented for a generic simulator framework. The postmortem trace analysis data is then fed into the visualization subsystem through a MySQL database. There is an overview visualization for execution traces of different components as small multiples, and a composite view of task view, component view, and legend bar. The composite view supports examining the usage of the GPUs in a hierarchical fashion, between GPU threads to the instruction. The composite view is effective in identifying #wavefronts executing in parallel in a compute unit at any given point in time. The lesser #wavefronts implies bottlenecks, and the tool helps in exploring the hierarchy to identify where improvement is needed. The tool is quite useful for hardware engineers to track the performance of the GPUs in today’s ever-increasing presence of GPUs in computational applications. To my knowledge, there are no other such comprehensive tools. The demo video and the user study demonstrate the intuitive usability of the tool.

This design study is complete and well-presented. Hence, my rating for acceptance.

My comments below are based on a few gaps I spotted, addressing which may strengthen the paper further.

Comments:
*********
The supplemental video is quite impressive. It elaborated on the problem statement and solution, along with a case study quite effectively. As mentioned in the paper, all the supplemental files, including source code is available at the bit.ly URL.

The paper mentions the usability of the Daisen across different GPU architecture has been taken care of by the use of generic simulator MGPUSim. It will be good to see a statement about the tool working with different GPUs. Perhaps, the GPUs used by the user study participants can be reported to strengthen the claim of the genericity.

It must be mentioned that the case study has been done for a postmortem trace analysis. There is a statement saying that “The same mechanism can be adopted for most computer architecture simulators or can capture live hardware executions.” Has Daisen been used on live hardware execution? If there is live/streaming data, there must be modifications in the backend server with respect to the updates and its periodicity. This needs to be mentioned.

It will be good to get a sense of what is the size of the data that gets stored in MySQL from the data gathered using the data collection library. What are also the estimates for the processing time of the data on the frontend server? Similarly what are the dataset sizes used for the user study, with reference to the statement: “In this process, they were asked to explore a dataset different from the onboarding tutorial”.

It’s gracious to mention the convenience sampling in the user study. However, there will always be a convenience bias owing to the user-base of this tool being domain-experts, and hence inherently biased. 

==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> survey.tex <==


% \section{A Survey Study of Performance Analysis}
% \label{sec:survey}

% To further motivate our work focusing on creating tools for computer architecture simulators, we conducted a survey study with \hl{37} computer architecture researchers who have experiences with computing system performance analysis. We created the survey using Google Forms and distributed via social media (e.g., Twitter, Slack) as well as academic conferences and workshops in the field of computer architecture in a convenience sample. We also conducted informal interviews with computer architecture researchers to identify design requirements and characterize practices and working flows around computer architecture simulators.
 
% \subsection{Survey Design}
% The survey contains three sections. The first section aimed to understand users' prior experience with performance analysis, particularly focusing on: how often respondents analyze computing system performance and use simulators during their daily work, how easy to identify and make sense of performance issues, and how much they feel the need tools to help them examine performance issues. This section contains seven items using a five-point scale. The choices range from (1) Strongly Disagree to (5) Strongly Agree.
% The second section of the survey aimed to help us characterize workflow and strategies. Questions were designed to understand simulators they have used and tools that help them identify performance issues, as well as to elaborate on the process of identify performance issues. This section contains four required free text questions and two multiple choices. 
% The last section included five questions that asked about respondents' position and affiliation, length of working on performance analysis, and whether or not they would be willing to be contacted for clarification questions.

% \subsection{Participants}

% 37 participants completed the survey as of March 2020. Since we used the convenience sampling for recruitment, it is likely to have potential bias of the sampling, such as under-representation of subpopulations in the sample. Therefore, more care should be taken to make inferences based on our convenience sample. We also avoid making absolute claims when analyzing and reporting our survey results. The aim of this survey is to examine the workflow of doing performance analysis and to help characterize domain tasks.   

% Participants had various working experience on performance analysis, ranging from less than a year (17.6\%), 1-2 years (17.6\%), 2-3 years (14.7\%), 3-5 years (23.5\%), 5-10 years (20.6\%), and over 10 years (5.9\%).
% A majority of them considered themselves doing computing system performance analysis as part of their job. More than half of them indicated that they had used computer architecture simulators in their daily work or study.

% \subsection{Survey Response Analysis}
% All responses were recorded via Google Forms and were kept in Google Sheets. We open coded \cite{thomas2006general} the comments and free-text answers to generate themes regarding the workflow of identifying performance and bottleneck issues. 

% The survey results show an apparent trend that computer architecture researchers need more tools to help them understand performance issues (41.2\% strongly agree, 38.2\% agree, 17.6\% neutral, 2.9\% disagree, 0\% strong disagree). 

% Strategies that researchers typically use to identify performance and bottleneck issues include gathering extra performance metrics (76.5\%), tuning parameters and running again to check how performance changes (64.7\%), making a guess of potential issues (58.8\%), and reading execution traces (58.8\%).

% We summarize challenges that researchers face with using existing tools for performance analysis. These challenges include: tools do not provide information they want (52.9\%), information is overwhelming and tools cannot provide an overview of performance problems (50.0\%), information is limited (47.1\%), information is too high-level and tools do not provide detailed information for reasoning (41.2\%), and difficulty in comparing amongst executions (14\%). 

